Asymmetric Tunneling of Bose-Einstein Condensates

In his celebrated textbook, $\textit{Quantum Mechanics: Nonrelativistic Theory}$, Landau argued that, for single particle systems in 1D, tunneling probability remains the same for a particle incident from the left or the right of a barrier. This left-right symmetry of tunneling probability holds regardless of the shape of the potential barrier. However, there are a variety of known cases that break this symmetry, e.g. when observing composite particles. We computationally (and analytically, in the simplest case) show this breaking of the left-right tunneling symmetry for Bose-Einstein condensates (BEC) in 1D, modelled by the Gross-Pitaevskii equation (GPE). By varying $g$, the parameter of inter-particle interaction in the BEC, we demonstrate that the transition from symmetric ($g=0$) to asymmetric tunneling is a threshold phenomenon. Our computations employ experimentally feasible parameters such that these results may be experimentally demonstrated in the near future. We conclude by suggesting applications of the phenomena to design atomtronic diodes, synthetic gauge fields, Maxwell's demons, and black-hole analogues.

==> Bin/abstract.tex <==
\begin{abstract}
Despite being uniquely quantum mechanical in nature, tunnelling is remarkably prolific effect found in many different fields of physics. While classical analogues do exist, the unique and unintuitive properties of tunneling still remain a source of study in physics today. For example, In his celebrated textbook, \textit{Quantum Mechanics-Nonrelativistic Theory}, Landau argued that, for single particle systems in 1D, tunneling probability remains the same for a particle incident from the left or the right. This left-right symmetry of tunneling probability holds regardless of the shape of the potential barrier, meaning that asymmetric barriers do not produce asymmetric tunneling. However, there a variety of known methods which may break this proposed symmetry, such as systems of composite particles. We set about proving Landau's original conjecture, as no rigorous proof currently exists. We then show the breaking of this predicted symmetry using Bose-Einstein condensates (BEC). Because, all particles of a BEC may inhabit the same quantum state, the system as a whole may be treated in most aspects as a single particle. However, BEC's are weakly interacting gases, and these weak, inter-atomic interaction preclude the use of the 1D, single particle Schr\"odinger equation. To this end, we use the Gross-Pitaevskii equation (GPE), a well known, nonlinear equation which accurately describes propagation of BEC's. By using the GPE to examine the 1D case of BEC's incident upon an asymmetric barrier, we demonstrate a method of breaking of left-right symmetry to quantum systems. Due to the wide-range of fields described using tunneling, these methods could be applied in many ways. Additionally, our method is designed to use experimentally implementable parameters such that these results may be proven in the near future.
%such as introducing phase decoherence using asymmetric potentials created by simple optical lattices. %this may be too much for abstract.
\end{abstract}
